The Topology-Free Construction of the Universal Type Structure for Conditional Probability Systems

We construct the universal type structure for conditional probability systems without any topological assumption, namely a type structure that is terminal, belief-complete, and non-redundant. In particular, in order to obtain the belief-completeness in a constructive way, we extend the work of Meier [An Infinitary Probability Logic for Type Spaces. Israel Journal of Mathematics, 192, 1-58] by proving strong soundness and strong completeness of an infinitary conditional probability logic with truthful and non-epistemic conditioning events.

==> Background/authors.tex <==
\author{Pierfrancesco Guarino\thanks{Maastricht University (AE1). \textit{E-mail:} \texttt{p.guarino@maastrichtuniversity.nl}.}}%

==> eptcsdata.tex <==
\providecommand{\firstpage}{285}
\providecommand{\publicationstatus}{J. Lang (Ed.): TARK 2017\\
EPTCS 251, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.251.20}{10.4204/EPTCS.251.20}}

